Voxgraph: Globally Consistent, Volumetric Mapping using Signed Distance Function Submaps

Globally consistent dense maps are a key requirement for long-term robot navigation in complex environments. While previous works have addressed the challenges of dense mapping and global consistency, most require more computational resources than may be available on-board small robots. We propose a framework that creates globally consistent volumetric maps on a CPU and is lightweight enough to run on computationally constrained platforms. Our approach represents the environment as a collection of overlapping Signed Distance Function (SDF) submaps, and maintains global consistency by computing an optimal alignment of the submap collection. By exploiting the underlying SDF representation, we generate correspondence free constraints between submap pairs that are computationally efficient enough to optimize the global problem each time a new submap is added. We deploy the proposed system on a hexacopter Micro Aerial Vehicle (MAV) with an Intel i7-8650U CPU in two realistic scenarios: mapping a large-scale area using a 3D LiDAR, and mapping an industrial space using an RGB-D camera. In the large-scale outdoor experiments, the system optimizes a 120x80m map in less than 4s and produces absolute trajectory RMSEs of less than 1m over 400m trajectories. Our complete system, called voxgraph, is available as open source.

==> bibliography_original.tex <==
@article{cadena2016past,
  title={Past, present, and future of simultaneous localization and mapping: Toward the robust-perception age},
  author={Cadena, Cesar and Carlone, Luca and Carrillo, Henry and Latif, Yasir and Scaramuzza, Davide and Neira, Jos{\'e} and Reid, Ian and Leonard, John J},
  journal={IEEE Transactions on robotics},
  volume={32},
  number={6},
  pages={1309--1332},
  year={2016},
  publisher={IEEE}
}

@inproceedings{burri2015real,
  title={Real-time visual-inertial mapping, re-localization and planning onboard mavs in unknown environments},
  author={Burri, Michael and Oleynikova, Helen and Achtelik, Markus W and Siegwart, Roland},
  booktitle={2015 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={1872--1878},
  year={2015},
  organization={IEEE}
}

@article{mur2015orb,
  title={ORB-SLAM: a versatile and accurate monocular SLAM system},
  author={Mur-Artal, Raul and Montiel, Jose Maria Martinez and Tardos, Juan D},
  journal={IEEE transactions on robotics},
  volume={31},
  number={5},
  pages={1147--1163},
  year={2015},
  publisher={IEEE}
}

@article{schneider2018maplab,
  title={maplab: An Open Framework for Research in Visual-inertial Mapping and Localization},
  author={T. Schneider and M. T. Dymczyk and M. Fehr and K. Egger and S. Lynen and I. Gilitschenski and R. Siegwart},
  journal={IEEE Robotics and Automation Letters},
  year={2018},
  doi={10.1109/LRA.2018.2800113}
}

@inproceedings{millane2018cblox,
  author={Millane, Alexander and Taylor, Zachary and Oleynikova, Helen and Nieto, Juan and Siegwart, Roland and Cadena, C{\'e}sar},
  booktitle={2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  title={C-blox: A Scalable and Consistent TSDF-based Dense Mapping Approach},
  year={2018}
}

@inproceedings{engel2014lsd,
  title={LSD-SLAM: Large-scale direct monocular SLAM},
  author={Engel, Jakob and Sch{\"o}ps, Thomas and Cremers, Daniel},
  booktitle={European conference on computer vision},
  pages={834--849},
  year={2014},
  organization={Springer}
}

@inproceedings{kerl2013dense,
  title={Dense visual SLAM for RGB-D cameras},
  author={Kerl, Christian and Sturm, J{\"u}rgen and Cremers, Daniel},
  booktitle={2013 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={2100--2106},
  year={2013},
  organization={IEEE}
}

@inproceedings{whelan2015elasticfusion,
  title={ElasticFusion: Dense SLAM without a pose graph},
  author={Whelan, Thomas and Leutenegger, Stefan and Salas-Moreno, R and Glocker, Ben and Davison, Andrew},
  organization={Robotics: Science and Systems},
  booktitle = {Robotics: {Science} and {Systems} {XI}},
  year={2015}
}

@inproceedings{whelan2012kintinuous,
  title={Kintinuous: Spatially extended kinectfusion},
  author={Whelan, Thomas and Kaess, Michael and Fallon, Maurice and Johannsson, Hordur and Leonard, John J and McDonald, John},
  year={2012},
  booktitle = {{AAAI} 2012},
}

@article{qin2018vins,
  title={Vins-mono: A robust and versatile monocular visual-inertial state estimator},
  author={Qin, Tong and Li, Peiliang and Shen, Shaojie},
  journal={IEEE Transactions on Robotics},
  volume={34},
  number={4},
  pages={1004--1020},
  year={2018},
  publisher={IEEE}
}

@article{hornung2013octomap,
  title={OctoMap: An efficient probabilistic 3D mapping framework based on octrees},
  author={Hornung, Armin and Wurm, Kai M and Bennewitz, Maren and Stachniss, Cyrill and Burgard, Wolfram},
  journal={Autonomous robots},
  volume={34},
  number={3},
  pages={189--206},
  year={2013},
  publisher={Springer}
}


@inproceedings{curless1996volumetric,
	title = {A volumetric method for building complex models from range images},
	doi = {10.1145/237170.237269},
	abstract = {A number of techniques have been developed for reconstructing surfaces by integrating groups of aligned range images. A desirable set of properties for such algorithms includes: incremental updating, representation of directional uncertainty, the ability to ﬁll gaps in the reconstruction, and robustness in the presence of outliers. Prior algorithms possess subsets of these properties. In this paper, we present a volumetric method for integrating range images that possesses all of these properties.},
	language = {en},
	booktitle = {Proceedings of the 23rd annual conference on {Computer} graphics and interactive techniques  - {SIGGRAPH} '96},
	publisher = {ACM Press},
	author = {Curless, Brian and Levoy, Marc},
	year = {1996},
	pages = {303--312}
}

@inproceedings{izadi2011kinectfusion,
  title={KinectFusion: real-time 3D reconstruction and interaction using a moving depth camera},
  author={Izadi, Shahram and Kim, David and Hilliges, Otmar and Molyneaux, David and Newcombe, Richard and Kohli, Pushmeet and Shotton, Jamie and Hodges, Steve and Freeman, Dustin and Davison, Andrew and others},
  booktitle={Proceedings of the 24th annual ACM symposium on User interface software and technology},
  pages={559--568},
  year={2011},
  organization={ACM}
}

@article{lin2018autonomous,
  title={Autonomous aerial navigation using monocular visual-inertial fusion},
  author={Lin, Yi and Gao, Fei and Qin, Tong and Gao, Wenliang and Liu, Tianbo and Wu, William and Yang, Zhenfei and Shen, Shaojie},
  journal={Journal of Field Robotics},
  volume={35},
  number={1},
  pages={23--51},
  year={2018},
  publisher={Wiley Online Library}
}

@inproceedings{oleynikova2017voxblox,
  title={Voxblox: Incremental 3d euclidean signed distance fields for on-board mav planning},
  author={Oleynikova, Helen and Taylor, Zachary and Fehr, Marius and Siegwart, Roland and Nieto, Juan},
  booktitle={2017 Ieee/rsj International Conference on Intelligent Robots and Systems (iros)},
  pages={1366--1373},
  year={2017},
  organization={IEEE}
}

@inproceedings{vempati2017onboard,
  title={Onboard real-time dense reconstruction of large-scale environments for UAV},
  author={Vempati, Anurag Sai and Gilitschenski, Igor and Nieto, Juan and Beardsley, Paul and Siegwart, Roland},
  booktitle={2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={3479--3486},
  year={2017},
  organization={IEEE}
}

@inproceedings{wagner2014graph,
  title={Graph SLAM with signed distance function maps on a humanoid robot},
  author={Wagner, Ren{\'e} and Frese, Udo and B{\"a}uml, Berthold},
  booktitle={2014 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={2691--2698},
  year={2014},
  organization={IEEE}
}

@article{oleynikova2018safe,
  title={Safe local exploration for replanning in cluttered unknown environments for microaerial vehicles},
  author={Oleynikova, Helen and Taylor, Zachary and Siegwart, Roland and Nieto, Juan},
  journal={IEEE Robotics and Automation Letters},
  volume={3},
  number={3},
  pages={1474--1481},
  year={2018},
  publisher={IEEE}
}

@article{niessner2013real,
  title={Real-time 3D reconstruction at scale using voxel hashing},
  author={Nie{\ss}ner, Matthias and Zollh{\"o}fer, Michael and Izadi, Shahram and Stamminger, Marc},
  journal={ACM Transactions on Graphics (ToG)},
  volume={32},
  number={6},
  pages={169},
  year={2013},
  publisher={ACM}
}

@article{dai2017bundlefusion,
  title={Bundlefusion: Real-time globally consistent 3d reconstruction using on-the-fly surface reintegration},
  author={Dai, Angela and Nie{\ss}ner, Matthias and Zollh{\"o}fer, Michael and Izadi, Shahram and Theobalt, Christian},
  journal={ACM Transactions on Graphics (ToG)},
  volume={36},
  number={3},
  pages={24},
  year={2017},
  publisher={ACM}
}

@article{maier2017efficient,
  title={Efficient online surface correction for real-time large-scale 3D reconstruction},
  author={Maier, Robert and Schaller, Raphael and Cremers, Daniel},
  journal={2017, British Machine Vision Conference (BMVC)},
  year={2017}
}

@inproceedings{wang2019real,
  title={Real-time Scalable Dense Surfel Mapping},
  author={Wang, Kaixuan and Gao, Fei and Shen, Shaojie},
  booktitle={2019 International Conference on Robotics and Automation (ICRA)},
  pages={6919--6925},
  year={2019},
  organization={IEEE}
}

@inproceedings{henry2013patch,
  title={Patch volumes: Segmentation-based consistent mapping with rgb-d cameras},
  author={Henry, Peter and Fox, Dieter and Bhowmik, Achintya and Mongia, Rajiv},
  booktitle={2013 International Conference on 3D Vision-3DV 2013},
  pages={398--405},
  year={2013},
  organization={IEEE}
}

@inproceedings{kahler2016real,
  title={Real-time large-scale dense 3D reconstruction with loop closure},
  author={K{\"a}hler, Olaf and Prisacariu, Victor A and Murray, David W},
  booktitle={European Conference on Computer Vision},
  pages={500--516},
  year={2016},
  organization={Springer}
}

@inproceedings{choi2015robust,
  title={Robust reconstruction of indoor scenes},
  author={Choi, Sungjoon and Zhou, Qian-Yi and Koltun, Vladlen},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5556--5565},
  year={2015}
}

@inproceedings{fioraio2015large,
  title={Large-scale and drift-free surface reconstruction using online subvolume registration},
  author={Fioraio, Nicola and Taylor, Jonathan and Fitzgibbon, Andrew and Di Stefano, Luigi and Izadi, Shahram},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4475--4483},
  year={2015}
}

@inproceedings{hess2016real,
  title={Real-time loop closure in 2D LIDAR SLAM},
  author={Hess, Wolfgang and Kohler, Damon and Rapp, Holger and Andor, Daniel},
  booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={1271--1278},
  year={2016},
  organization={IEEE}
}

@book{thrun2005probabilistic,
  title={Probabilistic robotics},
  author={Thrun, Sebastian and Burgard, Wolfram and Fox, Dieter},
  year={2005},
  publisher = {MIT Press},
}

@inproceedings{ratliff2009chomp,
  title={CHOMP: Gradient optimization techniques for efficient motion planning},
  author={Ratliff, Nathan and Zucker, Matt and Bagnell, J Andrew and Srinivasa, Siddhartha},
  year={2009},
  publisher={figshare},
  booktitle = {2009 {IEEE} {International} {Conference} on {Robotics} and {Automation}},
}

@inproceedings{han2018flashfusion,   
  title={FlashFusion: Real-time Globally Consistent Dense 3D Reconstruction using CPU computing}, 
  author={Lei, Han and Fang, Lu},   
  organization={Robotics: Science and Systems},   
  year={2018},
  booktitle = {Robotics: {Science} and {Systems}},
}

@article{GalvezTRO12,
  author={G\'alvez-L\'opez, Dorian and Tard\'os, J. D.},
  journal={IEEE Transactions on Robotics},
  title={Bags of Binary Words for Fast Place Recognition in Image Sequences},
  year={2012},
  month={October},
  volume={28},
  number={5},
  pages={1188--1197},
  doi={10.1109/TRO.2012.2197158},
  ISSN={1552-3098}
}

@book{christer_ericson_2005_collision-detection,
	address = {Amsterdam; Boston},
	series = {Morgan {Kaufmann} series in interactive 3D technology},
	title = {Real-time collision detection},
	isbn = {978-1-55860-732-3},
	publisher = {Elsevier},
	author = {{Christer Ericson}},
	year = {2005}
}

@article{lorensen_1987_marching-cubes,
	author = {Lorensen, William E. and Cline, Harvey E.},
	title = {Marching cubes: {A} high resolution 3D surface construction algorithm},
	shorttitle = {Marching cubes},
	journal = {SIGGRAPH},
	year = {1987}
}

@article{kiefer_1952_stochastic,
	author = {Kiefer, J. and Wolfowitz, J.},
	title = {Stochastic {Estimation} of the {Maximum} of a {Regression} {Function}},
	journal = {The Annals of Mathematical Statistics},
	year = {1952}
}

@incollection{burgard_2008_spatially-adaptive,
	author = {Burgard, W. and Brock, O. and Stachniss, C.},
	title = {Spatially-{Adaptive} {Learning} {Rates} for {Online} {Incremental} {SLAM}},
	booktitle = {Robotics: {Science} and {Systems} {III}},
	publisher = {MITP},
	year = {2008}
}

@inproceedings{olson_2006_fast-iterative,
	author = {Olson, E. and Leonard, J. and Teller, S.},
	title = {Fast iterative alignment of pose graphs with poor initial estimates},
	booktitle = {Proceedings 2006 {IEEE} {International} {Conference} on {Robotics} and {Automation}, 2006. {ICRA} 2006.},
	year = {2006}
}

@article{bloesch2017iterated,
  title={Iterated extended Kalman filter based visual-inertial odometry using direct photometric feedback},
  author={Bloesch, Michael and Burri, Michael and Omari, Sammy and Hutter, Marco and Siegwart, Roland},
  journal={The International Journal of Robotics Research},
  volume={36},
  number={10},
  pages={1053--1072},
  year={2017},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{zhang2018tutorial,
  title={A tutorial on quantitative trajectory evaluation for visual (-inertial) odometry},
  author={Zhang, Zichao and Scaramuzza, Davide},
  booktitle={2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={7244--7251},
  year={2018},
  organization={IEEE}
}

@article{zhang2017low,
  title={Low-drift and real-time lidar odometry and mapping},
  author={Zhang, Ji and Singh, Sanjiv},
  journal={Autonomous Robots},
  volume={41},
  number={2},
  pages={401--416},
  year={2017},
  publisher={Springer}
}

@inproceedings{zhang2015visual,
  title={Visual-lidar odometry and mapping: Low-drift, robust, and fast},
  author={Zhang, Ji and Singh, Sanjiv},
  booktitle={2015 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={2174--2181},
  year={2015},
  organization={IEEE}
}

@article{labbe2019rtab,
  title={RTAB-Map as an open-source lidar and visual simultaneous localization and mapping library for large-scale and long-term online operation},
  author={Labb{\'e}, Mathieu and Michaud, Fran{\c{c}}ois},
  journal={Journal of Field Robotics},
  volume={36},
  number={2},
  pages={416--446},
  year={2019},
  publisher={Wiley Online Library}
}

@book{kang_2006_color-technology,
	address = {Bellingham, Wash},
	title = {Computational color technology},
	isbn = {978-0-8194-6119-3},
	publisher = {SPIE Press},
	author = {Kang, Henry R.},
	year = {2006}
}

@article{dellaert2017factor,
  title={Factor graphs for robot perception},
  author={Dellaert, Frank and Kaess, Michael and others},
  journal={Foundations and Trends{\textregistered} in Robotics},
  volume={6},
  number={1-2},
  pages={1--139},
  year={2017},
  publisher={Now Publishers, Inc.}
}

@inproceedings{nikolic2014synchronized,
  title={A synchronized visual-inertial sensor system with FPGA pre-processing for accurate real-time SLAM},
  author={Nikolic, Janosch and Rehder, Joern and Burri, Michael and Gohl, Pascal and Leutenegger, Stefan and Furgale, Paul T and Siegwart, Roland},
  booktitle={2014 IEEE international conference on robotics and automation (ICRA)},
  pages={431--437},
  year={2014},
  organization={IEEE}
}

==> sections/acknowledgement.tex <==
\section*{Acknowledgment}

